Search for Light Neutral Bosons in the TREK/E36 Experiment at J-PARC

The Standard Model (SM) represents our best description of the subatomic world and it has been very successful in explaining how elementary particles interact under the influence of the fundamental forces. Despite its far reaching success in describing the building blocks of matter, the SM is still incomplete; falling short to explain dark matter, baryogenesis, neutrino masses and much more. The E36 experiment conducted at J-PARC in Japan, allows for sensitivity to search for light $U(1)$ gauge bosons, in the muonic $K^+$ decay channel. Such $U(1)$ bosons could be associated with dark matter or explain established muon-related anomalies such as the muon $g_{\mu}-2$ value, and the proton radius puzzle. A scintillating fiber target was used to stop a beam of positively charged $K$ mesons. The $K^+$ products were detected with a large-acceptance toroidal spectrometer capable of tracking charged particles with high resolution, combined with a large solid angle CsI(TI) photon detector and particle ID systems. A realistic simulation was employed to search for these rare decays in the mass range of 20$-$100 MeV/$c^2$. Preliminary results of the upper limits for the $A^\prime$ branching ratio $\mathcal{B}r(A^\prime)$ extracted at 95\% CL, will be discussed.

==> introduction.tex <==
\section{Introduction}
\label{intro}
 The primary goal of the TREK/E36 experiment was to provide a high precision electroweak measurement in order to test lepton universality, which is expressed as an identical coupling constant of the charged lepton family $(e,$ $\mu,$ and $\tau)$. Lepton universality is a staple of the Standard Model (SM) and any violation of this would be clear evidence of New Physics (NP) beyond the SM. E36 was designed to measure the ratio of the two-body decay widths $R_K=K_{e2}/K_{\mu2}$ with high precision. In the SM, the value of $R_K$ is very precise because to a first approximation the strong interaction dynamics cancel, leaving behind the expression \ref{eqn:ratioRk} \cite{Cirigliano:2007xi,e36prop}
 
 \begin{align}
  R^{SM}_{K}&=\frac{\Gamma(K^+\rightarrow e^+\nu_{e})}{\Gamma(K^+\rightarrow\mu^+\nu_{\mu})}\nonumber \\
  &=\frac{m^{2}_{e}}{m^{2}_{\mu}}\left(\frac{m^{2}_{K}-m^{2}_{e}}{m^{2}_{K}-m^{2}_{\mu}}\right)^2(1+\delta_r)\nonumber \\
  &=(2.477\pm0.001)\times10^{-5}
  \label{eqn:ratioRk}
 \end{align}

 \noindent where $m_K$, $m_e$ and $m_{\mu}$ are the masses of the $K^+$, $e^+$ and $\mu^+$, respectively, and $\delta_r$ represents radiative corrections corresponding to IB. Detailed calculations have been carried out in \cite{Cirigliano:2007ga}. This makes the SM value of $R^{SM}_{K}=2.477\times10^{-5}$ very accurate and enhanced sensitivity through helicity suppression makes it possible to search for NP effects by conducting a precise measurement of $R_K$ \cite{Cirigliano:2007xi}.
 
 Additionally, the TREK/E36 experiment is sensitive to searches for light neutral particles in the exotic kaon decay modes of $K^+\rightarrow\mu^+\nu_{\mu} A^{\prime}$ and/or $K^+\rightarrow\pi^+A^{\prime}$, followed by a prompt decay of the $A^{\prime}\rightarrow e^+e^-$. The former decay mode is of interest. This $A^{\prime}$, often dubbed a dark photon, could also be considered as a light neutral $U(1)$ boson, and might be a hidden force carrier of the dark sector associated with dark matter \cite{Bjorken:2009mm}. An $A^\prime$ that is weakly coupled to the SM and is sufficiently light could decay into observable electron-positron pairs, which can be used to reconstruct its invariant mass. Furthermore, the $A^\prime$ could help resolve, simultaneously, the proton radius puzzle and anomalous magnetic moment of the muon $g_{\mu}-2$ \cite{TuckerSmith:2010ra,Batell:2011qq,Carlson:2012pc,Carlson:2013mya}. Such hypothetic particles can also be conceived without violating existing constraints if they are fine-tuned and non-universally coupled \cite{Alanne:2020xcb,Fabbrichesi:2020wbt,Batell:2011qq,Carlson:2015poa,Carlson:2012pc,Carlson:2013mya}. In this case there would be a pronounced signal over the calculable SM leptonic radiative mode $K^+\rightarrow\mu^+\nu_{\mu}e^+e^-$ \cite{Carlson:2013mya,Carlson:2012pc}. Figure \ref{fig:kmuA} shows the Feynman diagram of muonic kaon decay involving an $A^\prime$ $K^+\rightarrow\mu^+\nu_{\mu}A^\prime$ followed promptly by $A^\prime\rightarrow e^+e^-$. 
 
 \begin{figure}[H]
  \begin{center}
   \includegraphics[scale=.95]{kmuAprime1.pdf}
   \includegraphics[scale=.95]{kmuAprime2.pdf}
   \caption{$A^{\prime}$ production amplitude. Feynman diagrams showing the channel of interest $K^{+}\rightarrow\mu^{+}\nu_{\mu}A^{\prime}$ \cite{Beranek:2012ey}.}
   \label{fig:kmuA}
  \end{center}
 \end{figure}

 Carlson and Rislow have calculated the branching ratio $\mathcal{B}r(K^+\rightarrow\mu^+\nu_{\mu}A^\prime)$ to be of order $10^{-5}$ for polar and axial vector couplings. Their prediction of the aforementioned branching ratio as a function of $m_{ee}$ indicates that a strong signal peak over the SM background would be observed experimentally in the invariant mass of the $e^+e^-$ par, $m_{ee}$, as shown in Figure \ref{fig:cmodel}\cite{Carlson:2013mya} for an assumed mass $m_{A\prime}=30$ MeV/$c^2$.
 
 \begin{figure}[H]
  \begin{center}
   \includegraphics[scale=.75]{carlsonModel1.pdf}
  \end{center}
  \caption{Strong signal to background prediction of the differential branching ratio as a function of $m_{ee}$. The QED background prediction for $K^{+}\rightarrow\mu^{+}\nu_{\mu}e^+e^-$ (red dashed curve) and the prediction with a 30 MeV/$c^2$ lepton universality violating $A^\prime$ of the Carlson model \cite{Carlson:2013mya}.}
  \label{fig:cmodel}
 \end{figure}

 Given the strong signal to background expectation of the Carlson model, the TREK/E36 experiment which is sensitive to light neutral bosons below 300 MeV would be able to test the efficacy of the Carlson model. The search would include a charged $\mu^+$ that is detected in the spectrometer gap and two clusters in the CsI barrel from $e^+e^-$ pairs, from which a peak search can be conducted in the invariant mass spectrum $m_{ee}$. 

